Table Space Designs For Implicit and Explicit Concurrent Tabled Evaluation

One of the main advantages of Prolog is its potential for the implicit exploitation of parallelism and, as a high-level language, Prolog is also often used as a means to explicitly control concurrent tasks. Tabling is a powerful implementation technique that overcomes some limitations of traditional Prolog systems in dealing with recursion and redundant sub-computations. Given these advantages, the question that arises is if tabling has also the potential for the exploitation of concurrency/parallelism. On one hand, tabling still exploits a search space as traditional Prolog but, on the other hand, the concurrent model of tabling is necessarily far more complex since it also introduces concurrency on the access to the tables. In this paper, we summarize Yap's main contributions to concurrent tabled evaluation and we describe the design and implementation challenges of several alternative table space designs for implicit and explicit concurrent tabled evaluation which represent different trade-offs between concurrency and memory usage. We also motivate for the advantages of using fixed-size and lock-free data structures, elaborate on the key role that the engine's memory allocator plays on such environments, and discuss how Yap's mode-directed tabling support can be extended to concurrent evaluation. Finally, we present our future perspectives towards an efficient and novel concurrent framework which integrates both implicit and explicit concurrent tabled evaluation in a single Prolog engine. Under consideration in Theory and Practice of Logic Programming (TPLP).

==> abstract.tex <==
One of the main advantages of Prolog is its potential for the implicit
exploitation of parallelism and, as a high-level language, Prolog is
also often used as a mean to explicitly control concurrent
tasks. Tabling is a powerful implementation technique that overcomes
some limitations of traditional Prolog systems in dealing with
recursion and redundant sub-computations. The question that arises is
if tabling has the potential for the exploitation of
concurrency/parallelism. Tabling exploits a search space as
traditional Prolog but, the concurrent model of tabling is necessarily
far more complex since it introduces concurrency on the access to the
tables. In this paper, we summarize Yap’s main contributions to
concurrent tabling and we describe the design and implementation
challenges of several alternative table space designs for implicit and
explicit concurrent tabling which represent different trade-offs
between concurrency and memory usage. We also motivate for the
advantages of using fixed-size and lock-free data structures,
elaborate on the key role that a memory allocator plays on such
environments, and discuss how Yap’s mode-directed tabling support can
be extended to concurrent evaluation. Finally, we present future
perspectives towards a novel framework which integrates
both implicit and explicit concurrent tabling in a single Prolog
engine.

